Vectorizing Projection in Manifold-Constrained Motion Planning for Real-Time Whole-Body Control

Many robot planning tasks require satisfaction of one or more constraints throughout the entire trajectory. For geometric constraints, manifold-constrained motion planning algorithms are capable of planning collision-free path between start and goal configurations on the constraint submanifolds specified by task. Current state-of-the-art methods can take tens of seconds to solve these tasks for complex systems such as humanoid robots, making real-world use impractical, especially in dynamic settings. Inspired by recent advances in hardware accelerated motion planning, we present a CPU SIMD-accelerated manifold-constrained motion planner that revisits projection-based constraint satisfaction through the lens of parallelization. By transforming relevant components into parallelizable structures, we use SIMD parallelism to plan constraint satisfying solutions. Our approach achieves up to 100-1000x speed-ups over the state-of-the-art, making real-time constrained motion planning feasible for the first time. We demonstrate our planner on a real humanoid robot and show real-time whole-body quasi-static plan generation. Our work is available at https://commalab.org/papers/mcvamp/.

==> cyclic_projection.tex <==
\begin{algorithm}[b]
\begin{footnotesize}
\caption{Cyclic Projection}
\label{alg:cyclicproject}
\begin{algorithmic}[1]
\Require $q_{s}, q_{g}, \text{constraints}$

\State $q_c \gets q_s$

\While{\textbf{true}}
    \State $d \gets 0$
    \For{$c \in \text{constraints}$}
        \State $d \gets d + \|c.\text{distanceToConstraint}(q_c)\|$
    \EndFor
    
    \If{$d < \textit{tol}$}
        \State \textbf{break}
    \EndIf
    
    \For{$c \in \text{constraints}$}
        \State $\text{step} \gets c.\text{getDescentStep}(q_c)$
        \State $q_c \gets q_c + \text{step}$
    \EndFor
\EndWhile

\State \Return $q_c$
\end{algorithmic}
\end{footnotesize}
\end{algorithm}


==> digit_constraints.tex <==
\begin{figure}[htbp]
    \centering
    \begin{tabular}{m{0.42\columnwidth} @{\hspace{0.05\columnwidth}} m{0.48\columnwidth}}
        
        \includegraphics[width=\linewidth,trim=1em 0em 1.5em 0.5em,clip]{images/digit/digit_constraints.jpg}

        & 
        \begin{minipage}{\linewidth}
            \centering
            \begin{tabular}{@{} l p{0.7\linewidth} @{}} %
                \toprule
                $\mathcal{C}_B$: & $T_{err} = T_{ref}^{-1}(T_L^{-1}T_R)$ \\
                                 & $d_B = \begin{bmatrix} t_{err} \\ \log(R_{err})^\vee \end{bmatrix}$ \\[0.8em]
                
                $\mathcal{C}_{CL}$: & $d_{CL} = \begin{bmatrix} \|X_{hip}^l - X_{tar}^l\| \\ \|X_{hip}^r - X_{tar}^r\| \end{bmatrix}$ \\[0.8em]
                
                $\mathcal{C}_{COM}$: & $d_{COM} = \mathbf{x}_{com}^{xy} - \mathrm{proj}(\mathbf{x}_{com}^{xy}, P)$ \\[0.8em]
                
                $\mathcal{C}_F$: & $d^f = \begin{bmatrix} t_{rel}^f \\ \log((T_{ref}^f)^{-1}T_f)^\vee \end{bmatrix}$ \\
                                 & $d_F = \begin{bmatrix} d^l & d^r \end{bmatrix}^\intercal$ \\
                \bottomrule
            \end{tabular}
        \end{minipage}
    \end{tabular}
\end{figure}

